Improving Visual Recognition with Hyperbolical Visual Hierarchy Mapping

Visual scenes are naturally organized in a hierarchy, where a coarse semantic is recursively comprised of several fine details. Exploring such a visual hierarchy is crucial to recognize the complex relations of visual elements, leading to a comprehensive scene understanding. In this paper, we propose a Visual Hierarchy Mapper (Hi-Mapper), a novel approach for enhancing the structured understanding of the pre-trained Deep Neural Networks (DNNs). Hi-Mapper investigates the hierarchical organization of the visual scene by 1) pre-defining a hierarchy tree through the encapsulation of probability densities; and 2) learning the hierarchical relations in hyperbolic space with a novel hierarchical contrastive loss. The pre-defined hierarchy tree recursively interacts with the visual features of the pre-trained DNNs through hierarchy decomposition and encoding procedures, thereby effectively identifying the visual hierarchy and enhancing the recognition of an entire scene. Extensive experiments demonstrate that Hi-Mapper significantly enhances the representation capability of DNNs, leading to an improved performance on various tasks, including image classification and dense prediction tasks.

==> rebuttal_table/compile_table.tex <==


\begin{table}[t]
    \centering
    \begin{subtable}[t]{0.49\linewidth}
        \caption{\textbf{Image classification on ImageNet-1K.}}
        \input{rebuttal_table/reb_big_cls} % 첫 번째 테이블
    \end{subtable}
    \begin{subtable}[t]{0.49\linewidth}
        \caption{\textbf{Semantic segmentation on ADE20K.}}
        \input{rebuttal_table/reb_big_seg} % 세 번째 테이블
    \end{subtable}
    % \begin{subtable}[t]{0.48\linewidth}
    %     \caption{\textbf{Human part segmentation on LIP.}}
    %     \input{rebuttal_table/reb_hierarchy_aware_recog} % 세 번째 테이블
    % \end{subtable}
    % \begin{subfigure}[t]
    %     \caption{\textbf{Human part segmentation on LIP.}}
    %     \includegraphics[width=0.45\linewidth]{rebuttal_table/graph.pdf} % 세 번째 테이블
    % \end{subfigure}
\end{table}
% \vspace{-5pt}


==> rebuttal_table/compile_table_fig.tex <==
\begin{figure}[t]
  \begin{minipage}[h]{.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{rebuttal_table/graph2.pdf}
  \end{minipage}\
  \begin{minipage}[h]{.45\linewidth}
    \centering
    \input{rebuttal_table/reb_hierarchy_aware_recog}
  \end{minipage}
\end{figure}

==> rebuttal_table/reb_big_cls.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\definecolor{LinkWater}{rgb}{0.854,0.882,0.949}
\label{tab:addlabel}
\scriptsize
\caption*{Table 1. {Classification on IN-1K.}}
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[330]Q[200]Q[200]Q[200]},
  cells = {c},
  row{3} = {LinkWater},
  row{5} = {LinkWater},
  vline{2} = {-}{},
  hline{1-2,6} = {-}{},}
Model            & Params & FLOPs & Top1 \\
Swin-S              & 50M    & 8.7G  & 83.0  \\
w/\textbf{VHM}  & 51M  & 9.0G  & 84.1  \\
DeiT-B              & 86M    & 17.6G & 81.8  \\
w/\textbf{VHM} & 87M  & 18.0G & 83.4  
\end{tblr}


==> rebuttal_table/reb_big_seg.tex <==

% \usepackage{color}
% \usepackage{tabularray}
\definecolor{LinkWater}{rgb}{0.847,0.882,0.949}
\definecolor{LinkWater1}{rgb}{0.85,0.882,0.949}
{\scriptsize
\label{tab:addlabel}
\caption*{Table 2. {Segmentation on ADE20K.}}
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[305]Q[217]Q[196]Q[169]},
  cells = {c},
  row{3} = {LinkWater},
  row{5} = {LinkWater},
  vline{2} = {-}{},
  hline{1-2,6} = {-}{},
}
Model            & Params & FLOPs & mIoU \\
Swin-S              & 81M    & 1038G & 47.6 \\
w/\textbf{VHM}  & 84M    & 1042G & 49.3 \\
DeiT-B              & 128M   & 1278G & 45.2 \\
w/\textbf{VHM} & 131M   & 1283G & 47.1 
\end{tblr}}


==> rebuttal_table/reb_hierarchy_aware_recog.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\definecolor{LinkWater}{rgb}{0.854,0.882,0.949}
\label{tab:addlabel}
{\scriptsize
\caption*{Table 3. {Part segmentation on LIP.}}
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[590]Q[160]Q[160]Q[160]},
  cells = {c},
  row{3} = {LinkWater},
  hline{1-2,4} = {-}{},
}
Method               & oAcc.    & mAcc           & mIoU           \\
PSPNet-50             & 0.788          & 0.551          & 0.461          \\
w/\textbf{VHM} & \textbf{0.798} & \textbf{0.570} & \textbf{0.477} 
\end{tblr}}


==> supple/algorithm.tex <==
\SetKwInput{KwRequire}{Require}
\label{sec:alg}
\vspace{-4pt}
\begin{algorithm}
    \caption{VHM Training.}
    \label{al_ppl}
    \LinesNumbered
    \KwRequire{The pre-trained image encoder $\mathcal{F}$, hierarchy decomposition module $\mathcal{D}$, and hierarchy encoder $\mathcal{G}$}
    \KwRequire{Initial level semantic seed distribution $\{\mathcal{N}(\mu_{c^{1}_{k}}, \sigma_{c^{1}_{k}})\}_{k=1}^{N}$ are randomly initialized}
    \KwRequire{Hyperbolic spaces \(\mathbb{L}\) initialized with curvature \(c=1\)}
    \While{Training}{
        Draw a mini-batch (\(I\), \(y\)).\\
        Sample initial semantic seeds \(\mathbf{c}^{1}\) from \(\{(\mu_{c^{1}_{k}}, \sigma_{c^{1}_{k}})\}_{k=1}^{N}\),\\
        Compute $v=\mathcal{F}(I)$ and semantic nodes \(\mathbf{s}^{1} = \mathcal{D}(v_{map}, \mathbf{c}^{1} )\) \\
        set \(l-1\) level as initial level\\
        \For{l to L}{
            Compute \(\{\mathcal{N}(\mu_{c^{l}_{k}}, \sigma_{c^{l}_{k}})\}_{k=1}^{N_{l}}\) according to Eq. (\red{})\\
            Sample \(\mathbf{c}^{l}\) from \(\{\mathcal{N}(\mu_{c^{l}_{k}}, \sigma_{c^{l}_{k}})\}_{k=1}^{N_{l}}\) according to Eq. (\red{})\\
            Compute \(l\) level semantic nodes \(\mathbf{s}^{l}\) according to Eq. (\red{})\\
            Compute representative semantic nodes \(\mathbf{s}^{l}_{k}\) according to Eq. (\red{})
        }
        \\
        Let $\boldsymbol{w}_{c}=\left[w_c^1,...,w_c^K\right] $\\
        Compute $\mathcal{L}_{div}$ according to Eq. (5)\\
        Compute $\boldsymbol{\sigma}_c^k=\mathcal{M}(w_{c}^k, v)$\\
        Compute $p(z|\boldsymbol{w}_c)$ according to Eq. (8)\\
        Compute $\mu(\boldsymbol{w}_c)$ and $\sigma(\boldsymbol{w}_c)$ according to Eq. (16), (17)\\
        Sample text embedding $\boldsymbol{z}_c$ from $p(z|\boldsymbol{w}_c)$\\
        Compute uncertainty $\log\sigma^2$ according to Eq. (18)\\
        Compute $\mathcal{L}_{KL}$ according to Eq. (12)\\
        Compute $\mathcal{L}_{pixel}$ according to Eq. (10)\\
        Compute $\mathcal{L}_{prob}$ according to Eq. (11)\\
        Compute total loss $\mathcal{L}$ according to Eq. (13)\\
        Update $\mathbf{P}$ and $\mathcal{M}$ by gradient descent\\}
\end{algorithm}

==> supple/compile_table.tex <==


\begin{table}[ht]
    \centering
    \begin{subtable}[t]{\linewidth}
        \centering
        \caption{\textbf{Quantitative results of image classification on ImageNet-1K.} with Swin-Tiny model~\cite{swin}}
        \input{supple/supple_cls} % 첫 번째 테이블
    \end{subtable}
    \hfill % 테이블 사이의 간격을 조정합니다.
    \begin{subtable}[t]{\linewidth}
        \centering
        \caption{\textbf{Quantitative results of object section and instance segmentation on COCO.} with Swin-Tiny model~\cite{swin}}
        \input{supple/supple_mask} % 두 번째 테이블
    \end{subtable}
    \hfill
    \begin{subtable}[t]{\linewidth}
        \centering
        \caption{\textbf{Quantitative results of semantic segmentation on ADE20K.} with Swin-Tiny model~\cite{swin}}
        \input{supple/supple_seg} % 세 번째 테이블
    \end{subtable}
\end{table}



==> supple/supple_cls.tex <==
% \usepackage{color}
% \usepackage{tabularray}
{\scriptsize
\label{tab:addlabel}
\begin{tblr}{
  colspec = {Q[367]Q[190]Q[171]Q[154]},
  cells = {c},
  row{4} = {LinkWater},
  cell{1}{1} = {r=2}{},
  hline{1,3,5} = {-}{},
}
Model                 & Params & FLOPs & Top-1         \\
                      & (M)    & (G)   & (\%)          \\
Swin-T                & 28.3   & 4.6   & 81.2          \\
\textbf{VHM}Swin-T & 29.5   & 4.9   & \textbf{83.4} 
\end{tblr}}



==> supple/supple_mask.tex <==
% \usepackage{color}
% \usepackage{tabularray}
{\scriptsize
\label{tab:addlabel}
\begin{tblr}{
  colspec = {Q[330]Q[130]Q[130]Q[130]Q[130]},
  cells = {c},
  row{4} = {LinkWater},
  cell{1}{1} = {r=2}{},
  cell{1}{4} = {r=2}{},
  cell{1}{5} = {r=2}{},
  hline{1,3,5} = {-}{},
}
Model              & Params & FLOPs & $AP^b$        & $AP^m$        \\
                   & (M)    & (G)   &               &               \\
Swin-T             & 48     & 267   & 42.7          & 39.3          \\
\textbf{VHM}Swin-T & 50     & 270   & \textbf{43.5} & \textbf{39.9} 
\end{tblr}}


==> supple/supple_seg.tex <==
% \usepackage{color}
% \usepackage{tabularray}
{\scriptsize
\label{tab:addlabel}
\begin{tblr}{
  colspec = {Q[350]Q[200]Q[130]Q[130]Q[130]},
  row{1} = {c},
  row{2} = {c},
  row{4} = {LinkWater},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{5} = {r=2}{},
  cell{3}{1} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{4}{1} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{4}{5} = {c},
  hline{1,3,5} = {-}{},
}
Model           & Method   & Params & FLOPs & mIoU          \\
                   &          & (M)    & (G)   &               \\
Swin-T             & UpderNet & 60     & 945.0 & 44.5          \\
\textbf{VHM}Swin-T & UpderNet & 62.1   & 948.3 & \textbf{46.8} 
\end{tblr}}


==> tab/table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
  \caption{Add caption}
    \begin{tabular}{ccccccc}
    \toprule
    \multicolumn{7}{c}{(a) Convolution model} \\
    \midrule
    \multicolumn{1}{l|}{Model} & \multicolumn{1}{l|}{Fine-tune} & \multicolumn{1}{l}{T-Params (M)} & \multicolumn{1}{l}{Params (M)} & \multicolumn{1}{l}{Flops(G)} & \multicolumn{1}{l|}{Input Size} & Top-1 \\
    \midrule
    RN50 & -     &       & 25M   & -     & -     & 80.4 \\
    \rowcolor[rgb]{ .816,  .808,  .808} \textbf{RN50-ours} & \textbf{H: 10 epochs} & 2.3   & 27M   & -     & -     & ongoing \\
    \midrule
    \multicolumn{7}{c}{(b) Transformer-Small models} \\
    \midrule
    \multicolumn{1}{l|}{Model} & \multicolumn{1}{l|}{Fine-tune} & \multicolumn{1}{l}{T-Params (M)} & \multicolumn{1}{l}{Params (M)} & \multicolumn{1}{l}{Flops(G)} & \multicolumn{1}{l|}{Input Size} & Top-1 \\
    \midrule
    DeiT-S & -     &       & 22    & 4.6   & 224   & 79.8 \\
    \rowcolor[rgb]{ .816,  .808,  .808} \textbf{DeiT-S-ours} & \textbf{H: 10 epochs} & 2.2   & 24    & 4.7   & 224   & 80.0(+0.2) \\
    \rowcolor[rgb]{ .949,  .949,  .949} \textbf{DeiT-S-ours} & F: 10 epochs & 24    & 24    & 4.7   & 224   & 80.3(+0.5) \\
    \midrule
    Swin-T & -     & -     & 29    & 4.5   & 224   & 82.2 \\
    \rowcolor[rgb]{ .816,  .808,  .808} \textbf{Swin-T-ours} & \textbf{H: 10 epochs} & 2.2   & 31    & 4.7   & 224   & 82.4(+0.2) \\
    \rowcolor[rgb]{ .949,  .949,  .949} \textbf{Swin-T-ours} & F: 10 epochs & 31    & 31    & 4.7   & 224   & ongoing \\
    \midrule
    \multicolumn{7}{c|}{(c) Transformer-Base models} \\
    \midrule
    \multicolumn{1}{l|}{Model} & \multicolumn{1}{l|}{Fine-tune} & \multicolumn{1}{l}{T-Params (M)} & \multicolumn{1}{l}{Params (M)} & \multicolumn{1}{l}{Flops(G)} & \multicolumn{1}{l|}{Input Size} & Top-1 \\
    \midrule
    Focal-B & -     &       & 90    & 16.4  & 224   & 83.8 \\
    \rowcolor[rgb]{ .816,  .808,  .808} \textbf{Focal-B-ours} & \textbf{H: 10 epochs} & 3.1   & 93    & 16.6  & 224   & ongoing \\
    \rowcolor[rgb]{ .949,  .949,  .949} \textbf{Focal-B-ours} & F: 10 epochs & 93    & 93    & 16.6  & 224   & ongoing \\
    \midrule
    Swin-S & -     &       & 50    & 8.7   & 224   & 83.0 \\
    \rowcolor[rgb]{ .816,  .808,  .808} \textbf{Swin-S-ours} & \textbf{H: 10 epochs} & 3.1   & 53    & 8.9   & 224   & ongoing \\
    \rowcolor[rgb]{ .949,  .949,  .949} \textbf{Swin-S-ours} & F: 10 epochs & 53    & 53    & 8.9   & 224   & ongoing \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%
\end{table*}%


==> tab/table2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \caption{Add caption}
    \begin{tabular}{cccccc}
    \toprule
    \multicolumn{6}{c}{(a) Convolution model} \\
    \midrule
    \multicolumn{1}{l|}{Model} & \multicolumn{1}{l|}{Fine-tune} & \multicolumn{1}{l}{Params (M)} & \multicolumn{1}{l}{Flops(G)} & \multicolumn{1}{l|}{Input Size} & Top-1 \\
    \midrule
    RNet-50 & -     & 25M   & -     & -     & 80.4 \\
    \rowcolor[rgb]{ .816,  .808,  .808} \textbf{RNet50-ours} & \textbf{50 epochs} & 27M   & -     & -     & 81.0(+0.6) \\
    \midrule
    \multicolumn{6}{c}{(b) Transformer(Small) models} \\
    \midrule
    \multicolumn{1}{l|}{Model} & \multicolumn{1}{l|}{Fine-tune} & \multicolumn{1}{l}{Params (M)} & \multicolumn{1}{l}{Flops(G)} & \multicolumn{1}{l|}{Input Size} & Top-1 \\
    \midrule
    DeiT-S & -     & 22    & 4.6   & 224   & 79.8 \\
    \rowcolor[rgb]{ .816,  .808,  .808} \textbf{DeiT-S-ours} & \textbf{50 epochs} & 24    & 4.7   & 224   & 80.3(+0.5) \\
    Swin-T & -     & 29    & 4.5   & 224   & 81.2 \\
    \rowcolor[rgb]{ .816,  .808,  .808} \textbf{Swin-T-ours} & \textbf{30 epochs} & 31    & 4.7   & 224   & 81.8(+0.6) \\
    \midrule
    \multicolumn{6}{c}{(c) Transformer(Base) models} \\
    \midrule
    \multicolumn{1}{l|}{Model} & \multicolumn{1}{l|}{Fine-tune} & \multicolumn{1}{l}{Params (M)} & \multicolumn{1}{l}{Flops(G)} & \multicolumn{1}{l|}{Input Size} & Top-1 \\
    \midrule
    DeiT-B & -     & 90    & 16.4  & 224   & 83.8 \\
    \rowcolor[rgb]{ .816,  .808,  .808} \textbf{DeiT-B-ours} & \textbf{50 epochs} & 93    & 16.6  & 224   & ongoing \\
    \midrule
    Swin-S & -     & 50    & 8.7   & 224   & 83.0 \\
    \rowcolor[rgb]{ .816,  .808,  .808} \textbf{Swin-S-ours} & \textbf{30 epochs} & 53    & 8.9   & 224   & ongoing \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> tab/table_finefull.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\begin{table}[t]
\centering
\caption{\textbf{Ablation studies} on \(v_{map}\) training methods. "Fine" and "Full" indicate "fine-tuning" and "full-training", respectively.}
\label{tab:ff}
{\scriptsize

\begin{tblr}{
  width = \linewidth,
  colspec = {Q[244]Q[169]Q[215]Q[119]Q[154]},
  row{1} = {c},
  cell{2}{2} = {c},
  cell{2}{3} = {c},
  cell{2}{4} = {c},
  cell{2}{5} = {c},
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{4}{2} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{4}{5} = {c},
  cell{5}{2} = {c},
  cell{5}{3} = {c},
  cell{5}{4} = {c},
  cell{5}{5} = {c},
  cell{6}{2} = {c},
  cell{6}{3} = {c},
  cell{6}{4} = {c},
  cell{6}{5} = {c},
  cell{7}{2} = {c},
  cell{7}{3} = {c},
  cell{7}{4} = {c},
  cell{7}{5} = {c},
  vline{2} = {-}{},
  hline{1,8} = {-}{0.15em},
  hline{2,5} = {-}{},
}
Model               & {Training\\Method} & {Top-1 Acc. \\(\%)} & {Flops\\(G)} & {Params\\(M)} \\
DeiT-Ti             & -                  & 72.2                & 1.3          & 5.7           \\
\textbf{VHM}DeiT-Ti & Fine               & \textbf{74.8(+2.6)} & 1.4          & 6.6           \\
\textbf{VHM}DeiT-Ti & Full               & 74.2(+2.0)          & 1.4          & 6.6           \\
DeiT-S              & -                  & 79.8                & 4.6          & 22            \\
\textbf{VHM}DeiT-S  & Fine               & 82.6(2.8)           & 4.7          & 23.4          \\
\textbf{VHM}DeiT-S  & Full               & \textbf{82.8(3.0)}  & 4.7          & 23.4          
\end{tblr}}
\end{table}

==> tab/table_hierst.tex <==
\definecolor{Mercury}{rgb}{0.901,0.898,0.898}
\begin{table}

\centering
\caption{Performance comparison for classification on ImageNet-1K~\cite{deng2009imagenet} according to the depth and width of the hierarchy tree.}\vspace{-5pt}
\label{tab:dw}
\resizebox{0.93\linewidth}{!}{
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[410]Q[171]Q[163]Q[171]},
  row{1} = {c},
  row{2} = {c},
  row{3} = {c},
  row{4} = {c},
  column{even} = {c},
  column{3} = {c},
  cell{2}{3} = {LinkWater},
  cell{4}{3} = {LinkWater},
  hline{1,3,5} = {-}{1pt},
  hline{2,4} = {-}{},
}
Hierarchy Width     &   16   &    32   &  64 \\                                                         
Top-1(\%)                                                               & 82.3 & 82.6 & 82.1 \\
Hierarchy Depth    &   3   &        4       &   5   \\
Top-1(\%)      & 82.4 & 82.6 & 82.3 
\end{tblr}}\vspace{-10pt}
\end{table}




==> talk.tex <==
% Hierarchical encoding procedure  
% 님님 ㅇㅇ
% 첫문단에 하고자하는말이 뭐야
% 1. DNNs의 distinctive feature representations
% 2. DNNs + hierarchical encoding process
% 3. hierarchical encoding process의 문제점과 그 한계
%     1. hierarchy within images.
%     2. hierachy among the semantic parts and their dependencies.1. DNNs의 distinctive feature representations
% 2. DNNs + hierarchical encoding process
% 3. hierarchical encoding process의 문제점과 그 한계
%     1. hierarchy within images.
%     2. hierachy among the semantic parts and their dependencies.
% 이건 참고 대충정리한거임
% 내가 생각하는 첫문단에 들어갈 내용 맞는지 봐바
% CNN은 convolution 쭉 진행하면서 hierarchy property 저절로 갖게되고
% vit는 hierchical encoding process가 없어서 swin 이런애들이 추가적으로 property 입력해주잖아 ㅇㅇ
% 맞지? ㅇㅇ
% 그럼 쓰는 순서를 
% DNN은 discriminative feature learning에 성공햇다
% 그 이유중 가장 중요하게 차지하는 부분중 하나가 hierarchy property이고
% CNNs의 hierarchy property는 어쩌구저쩌구
% VIT는 그런게 없어서 et al 들이 어쩌구저쩌구 해서 hierarchy encoding햇다
% 이렇게 진행할까?
% 두번째 문단?
% 지금 쓰고있는 방향이 뭔데?? 기존 hierarchical encoding방법 문제점 쓴거 아니야?
% 근데 hyperbolic말고도 cnn은 애초에 hierarchical property 존재하고 ViT with alpha components들도 hierarchy property 갖고있는데
% 얘네가 부족한 이유 먼저 설명해야되지 않아?
% 흠 괜찮은듯
% 근데 그 다음이 어떻게 해야할지 감이안잡히는데 
% 들어갈 수 있는 내용이
% hierarchy를 찾는데는 hyperbolic deep learning이 널리 쓰인다 > 하지만, remains~~~ > 우리방법
% 인데 hierarchy within image 이 부부분에 대한 부연설명이 부족함
% % 그 내용이 압축된게 이 아래문장임
% 아아 오키옼이
% 그러고 나서 hyperbolic 쓰고 오빠 방법 설명하겟다고??
% 그렇게 생각했는데 저 hyperbolic deep learning 이후에 내 방법을 설명하면 however이 너무 글에 많이 들어가는 느낌이라 뭔가 그냥 내방법에 대한 부연설명으로 넣어야하나 싶기도함
% hyperbolic을?흠 ㅇㅇㅇ
% 고러니께 글 전개가 hyperbolic manifolds를 사용하여 hierarchy를 많이 찾아왔음 하지만, 나 같은 방법은 없음 이랑
% 난 위에꺼가 나은거같은데 무적권 안까이게
% 흐으으으으으응ㅁ 일단 옼이ㅗㅋ이 오빠 고민이 뭔지 알갔음 생각해보겟음ㅋㅋㅋㅋㅎㅇㅌ
% 나도 그게 깔끔하긴한데 뭔가 문제점이 두개 같지않음? DNNs의 문제점이랑 기존 hyperbolic space의 활용부족을 동시에 짚는 것 같아서
% hierarcy찾는데 최적화된방법이 hyperbolic임 이런 측면에서 나는 ~~~를 제안함 중 못고르는중 
%나는 그앞에 쓰고 있어야지다시ㅋㅋㅋㅋㅋㅋ

% To address the problem, 
% Recently, hyperbolic deep learning has received a lot of attention for discovering the inherent hierarchy of data structures.
% Hence, the natural way to solve the aforementioned problem is to discover the hierarchical relationships in the final feature embedding space.
% Since acquiring annotation of hierarchy for given images is labor-intensive, we employ hyperbolic manifolds as embedding spaces for hierarchy
% In this paper
% In this regard, our approach focuses on discovering the intrinsic hierarchy within images, a task made challenging by the absence of explicit hierarchy annotations and the variable structure of components in terms of quantity, depth, and breadth across different images.
% To address this, we employ a strategy that not only discerns but also integrates these diverse hierarchical relationships within a unified feature space. 
% This methodology is designed to enhance the representation learning process, ensuring that the hierarchical structure is preserved and reflected in the final feature embeddings, thus facilitating a range of vision tasks from image classification to dense prediction.
% To utilize hierarchical relationships within the given images, we prop
% To overcome the aforementioned problem, we 
% However, since the hierarchical encoding process is conducted on gradually changing feature spaces, it is challenging to leverage the hierarchical relationships among the biggest semantic parts and their dependencies.
% In order to explore the hierarchy within the images with no additional annotations for hierarchy, 
% Over the decades, deep neural networks (DNNs), including convolutional neural networks (CNNs) and vision transformers (ViT), have seen tremendous advancements in various vision tasks. 
% This success is often attributed to pre-training on image classification tasks, where DNNs learn robust and distinctive feature representations.
% In addition to achieving distinct feature representations, there has been a focus on the architectural nuances of DNNs to allow for more granular feature representation. 
% A significant aspect of this is the hierarchical encoding procedure.
% In this context, due to their inherent properties, such as the sliding-window approach and local receptive fields, CNNs naturally undergo hierarchical encoding. 
% For instance, earlier layers in CNNs typically provide structural feature maps, while deeper layers capture more semantic features.
